Learning Pareto manifolds in high dimensions: How can regularization help?

Simultaneously addressing multiple objectives is becoming increasingly important in modern machine learning. At the same time, data is often high-dimensional and costly to label. For a single objective such as prediction risk, conventional regularization techniques are known to improve generalization when the data exhibits low-dimensional structure like sparsity. However, it is largely unexplored how to leverage this structure in the context of multi-objective learning (MOL) with multiple competing objectives. In this work, we discuss how the application of vanilla regularization approaches can fail, and propose a two-stage MOL framework that can successfully leverage low-dimensional structure. We demonstrate its effectiveness experimentally for multi-distribution learning and fairness-risk trade-offs.

==> AISTATS/tikz/lines.tex <==
\begin{tikzpicture}
  % First curve
  \node[label=left:{$\betastar$}] (N1) at (0,0){};
  \node[] (N2) at (4,0){};
  \draw[thick] (N1) .. controls (1,2) and (3,2) .. (N2);
  \fill (N1) circle (2pt);
  \fill (N2) circle (2pt);

  % Second curve, parallel to the first
  \node[] (N3) at (0,0.5){};
  \node[] (N4) at (4,0.5){};
  \draw[thick] (N3) .. controls (1,2.5) and (3,2.5) .. (N4);
  \fill (N3) circle (2pt);
  \fill (N4) circle (2pt);
\end{tikzpicture}
